SABAF: Removing Strong Attribute Bias from Neural Networks with Adversarial Filtering

Ensuring a neural network is not relying on protected attributes (e.g., race, sex, age) for prediction is crucial in advancing fair and trustworthy AI. While several promising methods for removing attribute bias in neural networks have been proposed, their limitations remain under-explored. To that end, in this work, we mathematically and empirically reveal the limitation of existing attribute bias removal methods in presence of strong bias and propose a new method that can mitigate this limitation. Specifically, we first derive a general non-vacuous information-theoretical upper bound on the performance of any attribute bias removal method in terms of the bias strength, revealing that they are effective only when the inherent bias in the dataset is relatively weak. Next, we derive a necessary condition for the existence of any method that can remove attribute bias regardless of the bias strength. Inspired by this condition, we then propose a new method using an adversarial objective that directly filters out protected attributes in the input space while maximally preserving all other attributes, without requiring any specific target label. The proposed method achieves state-of-the-art performance in both strong and moderate bias settings. We provide extensive experiments on synthetic, image, and census datasets, to verify the derived theoretical bound and its consequences in practice, and evaluate the effectiveness of the proposed method in removing strong attribute bias.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
 
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -pdf \"$_[0]\"" );
    }
}

==> sections/pictures/Adult_conflict.tex <==
\begin{figure}[htbp]
        \centering
        \includegraphics[width=\linewidth]{sections/figures/eb1_balanced-eb2_balanced_TestAcc_supp.pdf}
        \caption{Accuracy of \emph{Bias-conflicting} testing set under different bias strengths in Adult.}
        \label{fig:EB_Adult_biasconflicting_supp}
\end{figure}




==> sections/pictures/IMDB_EB_comparison.tex <==
\begin{figure*}
    \centering % <-- added
    
      \subfloat[EB1 dominated by females aged 25-29 and males aged 40-44.]{\includegraphics[width=0.4\linewidth]{sections/figures/IMDB_comparison_EB1.pdf}\label{fig:IMDB_comparison_eb1}}\quad
      
      \subfloat[EB2 dominated by females aged 40-44 and males aged 25-29.]{\includegraphics[width=0.4\linewidth]{sections/figures/IMDB_comparison_EB2.pdf}\label{fig:IMDB_comparison_eb2}}\quad

\caption{Comparison of dominated groups in EB1 and EB2.}
\label{fig:IMDB_EB_comparison}
\end{figure*}

==> sections/pictures/IMDB_noisy_examples.tex <==
\begin{figure*}
    \centering % <-- added
    
      \subfloat[Examples taken from distance view.]{\includegraphics[width=0.4\linewidth]{sections/figures/IMDB_long_distance.pdf}\label{fig:IMDB_long_distance}}\quad
      
      \subfloat[Examples with two faces.]{\includegraphics[width=0.4\linewidth]{sections/figures/IMDB_two_identities.pdf}\label{fig:IMDB_two}}\quad


\caption{Noisy examples of IMDB for sex classification.}
\label{fig:IMDB_noisy}
\end{figure*}

==> sections/tables/Adult_all.tex <==
\begin{figure*}[htbp]
    \begin{minipage}{0.48\textwidth}
        \centering
        % \includegraphics[width=\linewidth]{sections/figures/eb1_balanced-balanced_Test Acc.pdf}
        \includegraphics[width=\linewidth]{sections/figures/eb1_balanced-balanced_Test Acc_supp.pdf}
        \caption{Accuracy of \emph{Unbiased} testing set under different bias strengths in Adult. As bias strength increases, the effectiveness of all methods without universal dataset sharply declines to baseline.}
        \label{fig:EB_Adult_unbiased}
    \end{minipage}%
    \hspace{0.3cm}
    \begin{minipage}{0.48\textwidth}
        \captionsetup{type=table}
        % \caption{Extreme bias in Adult.}
        \caption{Accuracy under extreme bias in Adult. In the case of extreme bias, all methods perform close to baseline, and are ineffective in mitigating attribute bias. Only when universal dataset is introduced, attribute bias is clearly mitigated.}
        \label{tab:Adult_mostEx}
        \centering
        \resizebox{1\textwidth}{!}{%
\begin{tabular}{lcc}
\toprule
                         & Unbiased            & Bias-conflicting    \\
                         \midrule
Baseline                 & 50.59{\scriptsize $\pm$ 0.54}          & 1.19{\scriptsize $\pm$ 0.83}           \\
LNL~\cite{learn_not_to_learn_Colored_MNIST}                       & 50.10{\scriptsize $\pm$ 0.18}          & 0.43{\scriptsize $\pm$ 0.46}          \\
% DR     $\star$                  & 66.38{\scriptsize $\pm$ 0.22}          & 38.17{\scriptsize $\pm$ 1.04}          \\
EnD~\cite{End}                      & 50.59{\scriptsize $\pm$ 0.75}          & 1.18{\scriptsize $\pm$ 0.96}           \\
CSAD~\cite{CSAD}                     & 50.76{\scriptsize $\pm$ 2.22}          & 1.43{\scriptsize $\pm$ 2.46}           \\
Ours                     & 50.09{\scriptsize $\pm$ 0.81}          & 0.64{\scriptsize $\pm$ 1.01}           \\
\midrule
Ours (Universal) & \textbf{74.93{\scriptsize $\pm$ 0.95}} & \textbf{57.63{\scriptsize $\pm$ 1.30}} \\
\bottomrule
\end{tabular}
        }
    \end{minipage}
\end{figure*}



==> sections/tables/CelebA_lambda_rec.tex <==
\begin{table}[htbp]
\caption{Average accuracy of \emph{Unbiased} testing set on all 23 non-sex-related downstream tasks of CelebA. Our filter is trained on extreme bias data (\emph{TrainEx} training set). The vanilla baseline performance is 59.03{\scriptsize $\pm$ 0.96}.}
\label{tab:CelebA_lambda_rec}
\centering
% \resizebox{0.7\textwidth}{!}{%
\begin{tabular}{lccccc}
\toprule
$\lambda_{rec}$ & 0        & 10       & 50       & 100      & 110      \\
\midrule
Ours                    & 35.92{\scriptsize $\pm$1.81} & 49.47{\scriptsize $\pm$1.33} & 55.14{\scriptsize $\pm$0.97} & \textbf{60.13{\scriptsize $\pm$0.27}} & 59.96{\scriptsize $\pm$0.18} \\
\bottomrule
\end{tabular}
% }
\end{table}

